Linking Datasets on Organizations Using Half A Billion Open-Collaborated Records

Scholars studying organizations often work with multiple datasets lacking shared identifiers or covariates. In such situations, researchers usually use approximate string ("fuzzy") matching methods to combine datasets. String matching, although useful, faces fundamental challenges. Even where two strings appear similar to humans, fuzzy matching often struggles because it fails to adapt to the informativeness of the character combinations. In response, a number of machine learning methods have been developed to refine string matching. Yet, the effectiveness of these methods is limited by the size and diversity of training data. This paper introduces data from a prominent employment networking site (LinkedIn) as a massive training corpus to address these limitations. By leveraging information from the LinkedIn corpus regarding organizational name-to-name links, we incorporate trillions of name pair examples into various methods to enhance existing matching benchmarks and performance by explicitly maximizing match probabilities. We also show how relationships between organization names can be modeled using a network representation of the LinkedIn data. In illustrative merging tasks involving lobbying firms, we document improvements when using the LinkedIn corpus in matching calibration and make all data and methods open source.

==> ExecutionTime4.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sun, Jun 16, 2024 - 07:39:09
\begin{table}[!htbp] \centering 
  \caption{Run time on the company lobbying data analysis.} 
  \label{tab:ExTime4} 
\begin{tabular}{@{\extracolsep{5pt}} cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Algorithm & Run Time (mins) \\ 
\hline \\[-1.8ex] 
Bipartite & 13.40 \\ 
Bipartite-ML & 318.44 \\ 
DeezyMatch & 0.32 \\ 
Fuzzy & 0.33 \\ 
Lookup & 1.36 \\ 
Markov & 9.47 \\ 
Markov-ML & 142.50 \\ 
ML & 2.09 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> ExecutionTime5.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sun, Jun 16, 2024 - 07:38:54
\begin{table}[!htbp] \centering 
  \caption{Run time on the cross-language merge task.} 
  \label{tab:ExTime5} 
\begin{tabular}{@{\extracolsep{5pt}} cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Algorithm & Run Time (mins) \\ 
\hline \\[-1.8ex] 
Bipartite & 0.70 \\ 
Bipartite-ML & 6.17 \\ 
DeezyMatch & 0.15 \\ 
Fuzzy & 0.02 \\ 
Lookup & 1.11 \\ 
Markov & 0.29 \\ 
Markov-ML & 3.52 \\ 
ML & 1.39 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> ExecutionTime7.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sun, Jun 16, 2024 - 07:39:17
\begin{table}[!htbp] \centering 
  \caption{Run time on the Y Combinator task.} 
  \label{tab:ExTime7} 
\begin{tabular}{@{\extracolsep{5pt}} cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Algorithm & Run Time (mins) \\ 
\hline \\[-1.8ex] 
Bipartite & 6.53 \\ 
Bipartite-ML & 143.80 \\ 
DeezyMatch & 0.31 \\ 
Fuzzy & 0.15 \\ 
Lookup & 1.24 \\ 
Markov & 4.48 \\ 
Markov-ML & 65.97 \\ 
ML & 1.35 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> ExecutionTime8.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sun, Jun 16, 2024 - 07:39:22
\begin{table}[!htbp] \centering 
  \caption{Run time on the Y Combinator task.} 
  \label{tab:ExTime8} 
\begin{tabular}{@{\extracolsep{5pt}} cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Algorithm & Run Time (mins) \\ 
\hline \\[-1.8ex] 
Bipartite & 7.63 \\ 
Bipartite-ML & 142.84 \\ 
DeezyMatch & 0.33 \\ 
Fuzzy & 0.15 \\ 
Lookup & 1.26 \\ 
Markov & 4.41 \\ 
Markov-ML & 66.16 \\ 
ML & 1.22 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

